Joint Embedding of Structural and Functional Brain Networks with Graph Neural Networks for Mental Illness Diagnosis

Multimodal brain networks characterize complex connectivities among different brain regions from both structural and functional aspects and provide a new means for mental disease analysis. Recently, Graph Neural Networks (GNNs) have become a de facto model for analyzing graph-structured data. However, how to employ GNNs to extract effective representations from brain networks in multiple modalities remains rarely explored. Moreover, as brain networks provide no initial node features, how to design informative node attributes and leverage edge weights for GNNs to learn is left unsolved. To this end, we develop a novel multiview GNN for multimodal brain networks. In particular, we regard each modality as a view for brain networks and employ contrastive learning for multimodal fusion. Then, we propose a GNN model which takes advantage of the message passing scheme by propagating messages based on degree statistics and brain region connectivities. Extensive experiments on two real-world disease datasets (HIV and Bipolar) demonstrate the effectiveness of our proposed method over state-of-the-art baselines.

==> sections/ethical-statements.tex <==
\section{Compliance with Ethical Standards}
The research work is related to human studies. The HIV and Bipolar datasets employed in this study are owned by a third-party organization, where informed consent was obtained for all subjects. The data processed is anonymous with no personally identifiable information. All studies are conducted according to the Good Clinical Practice guidelines and U.S. 21 CFR Part 50 (Protection of Human Subjects).

% \section{Acknowledgements}
% No funding was received for conducting this study. The authors have no relevant financial or non-financial interests to disclose.

